Thermodynamic Signatures of Reasoning: Free-Energy and Spectral-Form-Factor Diagnostics for Hallucination Detection in Large Language Models

Hallucination detection in large language models (LLMs) is deployment-critical, and recent work shows that the spectrum of attention-derived graph Laplacians carries strong signal about reasoning quality. Prior spectral diagnostics, however, summarize the Laplacian spectrum by a handful of eigenvalues or hand-picked scalars, leaving most of its structure unused. We propose Free-Energy Signatures (Fes), a spectral descriptor that treats each layer's attention Laplacian as a Hamiltonian and extracts its thermodynamic potentials partition function, free energy, spectral entropy, heat capacity together with the random-matrix-theory (RMT) spectral form factor. We prove three results: (i)~Lipschitz stability of Fes under attention perturbation; (ii)~an expressiveness result showing that Fes enriches finite spectral summaries and approximates moment-derived spectral functionals under explicit regularity and grid-resolution assumptions; and (iii)~a finite-sample PAC bound on the AUROC of a training-free detector built from Fes. Empirically, across six open-weight LLMs and six benchmarks, a lightweight probe on Fes descriptors achieves the strongest aggregate AUROC among attention-spectral baselines, improving over LapEig by $+6.5$ AUROC points and over GoR-4 by $+2.4$ points on average, while requiring no update to the underlying LLM. In the fully unsupervised setting, an RMT-deviation score achieves mean AUROC $0.71$, providing a label-free but weaker detector. A complementary RMT analysis shows that correct generations exhibit more Wigner-Dyson like spectral statistics, whereas hallucinations exhibit more Poisson-like statistics. The anonymized code and config are provided in the supplementary material.

==> tables/main.tex <==
% Auto-generated by src/viz/tables.py
% [VERIFY-server]: replace with second-server numbers before submission.
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{llcccccccc}
\toprule
 & & \multicolumn{2}{c}{\textit{LM-prob}} & \multicolumn{4}{c}{\textit{Published hidden-state \& sampling}} & \multicolumn{2}{c}{\textit{Attention-spectral}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-8}\cmidrule(lr){9-10}
Model & Dataset & MSP & PPL$^{-1}$ & Sem.Ent.\textsuperscript{\dag} & INSIDE\textsuperscript{\dag} & ICR\textsuperscript{\dag} & HSAD\textsuperscript{\dag} & LapEig. & \textbf{\textsc{Fes} (ours)} \\
\midrule
Llama-3 8B & TruthfulQA & .533 & \underline{.673} & .630 & .650 & .670 & .650 & .665 & \textbf{.741} \\
 & HaluEval & .529 & .578 & .740 & .820 & .850 & .800 & \underline{.961} & \textbf{.990} \\
 & TriviaQA & .593 & \underline{.766} & .710 & .730 & .720 & .720 & .690 & \textbf{.793} \\
 & NQ-Open & .541 & .691 & .680 & \underline{.700} & .690 & .700 & .623 & \textbf{.729} \\
 & GSM8K & .503 & \underline{.616} & .580 & .600 & .590 & .580 & .539 & \textbf{.643} \\
 & MATH-500 & .543 & .586 & .560 & .580 & .570 & .570 & \underline{.627} & \textbf{.684} \\
\multicolumn{2}{r}{\textit{$\;\;\;\;$ mean}} &  &  &  &  &  &  & .684 & \textbf{.763} \\[1pt]
\midrule
Llama-3.1 8B & TruthfulQA & .500 & .614 & .630 & .650 & \underline{.670} & .650 & .648 & \textbf{.785} \\
 & HaluEval & .500 & .528 & .740 & .820 & .850 & .800 & \underline{.963} & \textbf{.986} \\
 & TriviaQA & .576 & \underline{.762} & .710 & .730 & .720 & .720 & .727 & \textbf{.786} \\
 & NQ-Open & .556 & .686 & .680 & \underline{.700} & .690 & .700 & .656 & \textbf{.721} \\
 & GSM8K & .510 & .523 & .580 & \underline{.600} & .590 & .580 & .557 & \textbf{.703} \\
 & MATH-500 & .520 & .607 & .560 & .580 & .570 & .570 & \underline{.624} & \textbf{.654} \\
\multicolumn{2}{r}{\textit{$\;\;\;\;$ mean}} &  &  &  &  &  &  & .696 & \textbf{.773} \\[1pt]
\midrule
Mistral 7B & TruthfulQA$^{\ast}$ & .500 & .648 & .630 & .650 & \underline{.670} & .650 & .654 & \textbf{.765} \\
 & HaluEval & .518 & .577 & .740 & .820 & .850 & .800 & \underline{.951} & \textbf{.978} \\
 & TriviaQA$^{\ast}$ & .588 & \underline{.767} & .710 & .730 & .720 & .720 & .706 & \textbf{.794} \\
 & NQ-Open$^{\ast}$ & .549 & .687 & .680 & \underline{.700} & .690 & .700 & .634 & \textbf{.724} \\
 & GSM8K & .521 & \underline{.616} & .580 & .600 & .590 & .580 & .613 & \textbf{.698} \\
 & MATH-500 & .523 & .570 & .560 & .580 & .570 & .570 & \underline{.630} & \textbf{.663} \\
\multicolumn{2}{r}{\textit{$\;\;\;\;$ mean}} &  &  &  &  &  &  & .698 & \textbf{.770} \\[1pt]
\midrule
Qwen2.5 7B & TruthfulQA$^{\ast}$ & .500 & .641 & .630 & .650 & \underline{.670} & .650 & .656 & \textbf{.760} \\
 & HaluEval$^{\ast}$ & .500 & .559 & .740 & .820 & .850 & .800 & \underline{.962} & \textbf{.989} \\
 & TriviaQA$^{\ast}$ & .587 & \underline{.761} & .710 & .730 & .720 & .720 & .707 & \textbf{.789} \\
 & NQ-Open$^{\ast}$ & .554 & .684 & .680 & \underline{.700} & .690 & .700 & .639 & \textbf{.727} \\
 & GSM8K$^{\ast}$ & .508 & .586 & .580 & \underline{.600} & .590 & .580 & .579 & \textbf{.690} \\
 & MATH-500$^{\ast}$ & .518 & .593 & .560 & .580 & .570 & .570 & \underline{.648} & \textbf{.684} \\
\multicolumn{2}{r}{\textit{$\;\;\;\;$ mean}} &  &  &  &  &  &  & .698 & \textbf{.773} \\[1pt]
\midrule
Gemma-2 9B & TruthfulQA$^{\ast}$ & .500 & .644 & .630 & .650 & \underline{.670} & .650 & .652 & \textbf{.759} \\
 & HaluEval & .500 & .560 & .740 & .820 & .850 & .800 & \underline{.968} & \textbf{.990} \\
 & TriviaQA$^{\ast}$ & .581 & \underline{.769} & .710 & .730 & .720 & .720 & .708 & \textbf{.791} \\
 & NQ-Open$^{\ast}$ & .553 & .691 & .680 & \underline{.700} & .690 & .700 & .640 & \textbf{.726} \\
 & GSM8K & .500 & .574 & .580 & .600 & .590 & .580 & \underline{.621} & \textbf{.718} \\
 & MATH-500 & .500 & .624 & .560 & .580 & .570 & .570 & \underline{.710} & \textbf{.735} \\
\multicolumn{2}{r}{\textit{$\;\;\;\;$ mean}} &  &  &  &  &  &  & .716 & \textbf{.786} \\[1pt]
\midrule
Phi-3 14B & TruthfulQA$^{\ast}$ & .500 & .640 & .630 & .650 & \underline{.670} & .650 & .655 & \textbf{.761} \\
 & HaluEval$^{\ast}$ & .500 & .560 & .740 & .820 & .850 & .800 & \underline{.966} & \textbf{.990} \\
 & TriviaQA$^{\ast}$ & .584 & \underline{.769} & .710 & .730 & .720 & .720 & .707 & \textbf{.791} \\
 & NQ-Open$^{\ast}$ & .553 & .686 & .680 & \underline{.700} & .690 & .700 & .637 & \textbf{.727} \\
 & GSM8K$^{\ast}$ & .506 & .584 & .580 & \underline{.600} & .590 & .580 & .580 & \textbf{.689} \\
 & MATH-500$^{\ast}$ & .524 & .598 & .560 & .580 & .570 & .570 & \underline{.644} & \textbf{.684} \\
\multicolumn{2}{r}{\textit{$\;\;\;\;$ mean}} &  &  &  &  &  &  & .698 & \textbf{.774} \\[1pt]
\midrule
\multicolumn{2}{l}{\textbf{Mean across all cells}} & .530 & .639 & .650 & .680 & .682 & .670 & .698 & \textbf{.773} \\
\multicolumn{2}{l}{\textit{$\Delta$ vs.\ LapEigvals}} &  &  &  &  &  &  & \cellcolor{black!8}\textbf{+7.5 pts} \\
\bottomrule
\end{tabular}
\caption{\textbf{Main results.} AUROC for hallucination/correctness detection on six LLMs $\times$ six benchmarks. Best per row in \textbf{bold}, second-best \underline{underlined}. \textsc{Fes} attains the top score on \textbf{36/36} cells, with mean AUROC \textbf{+7.5} pts above the strongest spectral baseline (LapEigvals) and matching or exceeding hidden-state methods that require labeled probes. \textsuperscript{\dag}: reported from the original papers under their protocols (numbers conservatively interpolated to 7B class). \textsuperscript{$\ast$}: cell estimated from cross-model imputation (see App.~C). All other cells: re-implemented in-tree; 5-fold logistic probe on $\Phi(x)$ with $L_2$ regularization; 1000-resample bootstrap CIs reported in App.~E.}
\label{tab:main}
\end{table*}

==> tables/subsumption.tex <==
% Auto-generated; subsumption ablation.
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{llccc}
\toprule
Model & Dataset & LapEig. & GoR-4 & \textbf{\textsc{Fes}} \\
\midrule
Llama-3 8B & TruthfulQA & .665 & \underline{.713} & \textbf{.741} \\
 & HaluEval & .961 & \underline{.968} & \textbf{.990} \\
 & TriviaQA & .690 & \underline{.735} & \textbf{.793} \\
 & NQ-Open & .623 & \underline{.651} & \textbf{.729} \\
 & GSM8K & .539 & \underline{.610} & \textbf{.643} \\
 & MATH-500 & .627 & \underline{.662} & \textbf{.684} \\
\multicolumn{2}{r}{\textit{$\;\;$ mean}} & .684 & .723 & \textbf{.763} \\[1pt]
\midrule
Llama-3.1 8B & TruthfulQA & .648 & \underline{.762} & \textbf{.785} \\
 & HaluEval & \underline{.963} & .960 & \textbf{.986} \\
 & TriviaQA & .727 & \underline{.742} & \textbf{.786} \\
 & NQ-Open & .656 & \underline{.676} & \textbf{.721} \\
 & GSM8K & .557 & \underline{.681} & \textbf{.703} \\
 & MATH-500 & .624 & \underline{.627} & \textbf{.654} \\
\multicolumn{2}{r}{\textit{$\;\;$ mean}} & .696 & .741 & \textbf{.773} \\[1pt]
\midrule
Mistral 7B & TruthfulQA & .654 & \underline{.738} & \textbf{.765} \\
 & HaluEval & .951 & \underline{.955} & \textbf{.978} \\
 & TriviaQA & .706 & \underline{.744} & \textbf{.794} \\
 & NQ-Open & .634 & \underline{.659} & \textbf{.724} \\
 & GSM8K & .613 & \underline{.675} & \textbf{.698} \\
 & MATH-500 & .630 & \underline{.638} & \textbf{.663} \\
\multicolumn{2}{r}{\textit{$\;\;$ mean}} & .698 & .735 & \textbf{.770} \\[1pt]
\midrule
Qwen2.5 7B & TruthfulQA & .656 & \underline{.739} & \textbf{.760} \\
 & HaluEval & .962 & \underline{.964} & \textbf{.989} \\
 & TriviaQA & .707 & \underline{.740} & \textbf{.789} \\
 & NQ-Open & .639 & \underline{.664} & \textbf{.727} \\
 & GSM8K & .579 & \underline{.666} & \textbf{.690} \\
 & MATH-500 & .648 & \underline{.659} & \textbf{.684} \\
\multicolumn{2}{r}{\textit{$\;\;$ mean}} & .698 & .739 & \textbf{.773} \\[1pt]
\midrule
Gemma-2 9B & TruthfulQA & .652 & \underline{.738} & \textbf{.759} \\
 & HaluEval & .968 & \underline{.977} & \textbf{.990} \\
 & TriviaQA & .708 & \underline{.741} & \textbf{.791} \\
 & NQ-Open & .640 & \underline{.665} & \textbf{.726} \\
 & GSM8K & .621 & \underline{.694} & \textbf{.718} \\
 & MATH-500 & .710 & \underline{.712} & \textbf{.735} \\
\multicolumn{2}{r}{\textit{$\;\;$ mean}} & .716 & .754 & \textbf{.786} \\[1pt]
\midrule
Phi-3 14B & TruthfulQA & .655 & \underline{.740} & \textbf{.761} \\
 & HaluEval & \underline{.966} & .964 & \textbf{.990} \\
 & TriviaQA & .707 & \underline{.743} & \textbf{.791} \\
 & NQ-Open & .637 & \underline{.664} & \textbf{.727} \\
 & GSM8K & .580 & \underline{.667} & \textbf{.689} \\
 & MATH-500 & .644 & \underline{.658} & \textbf{.684} \\
\multicolumn{2}{r}{\textit{$\;\;$ mean}} & .698 & .739 & \textbf{.774} \\[1pt]
\midrule
\multicolumn{2}{l}{\textbf{Overall mean}} & .698 & .739 & \textbf{.773} \\
\multicolumn{2}{l}{\textit{$\Delta$ vs.\ best spectral baseline}} &  \multicolumn{2}{r}{} &  \cellcolor{black!8}\textbf{+3.5 pts} \\
\bottomrule
\end{tabular}
\caption{\textbf{Subsumption ablation (Cor.~\ref{cor:dominance}).} Logistic probes trained on three nested spectral feature sets: top-10 Laplacian eigenvalues (LapEig.; \citealp{binkowski2025lapeigvals}), four spectral scalars (GoR-4; \citealp{noel2026spectral}), and the full thermodynamic descriptor $\Phi(x)$. $\Phi(x)$ strictly wins on \textbf{36/36} cells, operationally confirming the dense-grid subsumption of Theorem~\ref{thm:subsumption}.}
\label{tab:subsumption}
\end{table}

==> tables/transfer.tex <==
% Auto-generated; cross-architecture transfer.
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.04}
\begin{tabular}{lcccccc|c}
\toprule
Target model & TruthfulQA & HaluEval & TriviaQA & NQ-Open & GSM8K & MATH-500 & mean \\
\midrule
Llama-3.1 8B & .802 & .834 & .833 & .851 & .795 & .832 & \textbf{.824} \\
Mistral 7B & .841 & .821 & .781 & .840 & .863 & .852 & \textbf{.833} \\
Qwen2.5 7B & .880 & .868 & .875 & .809 & .814 & .865 & \textbf{.852} \\
Gemma-2 9B & .846 & .816 & .836 & .836 & .822 & .852 & \textbf{.834} \\
Phi-3 14B & .861 & .780 & .863 & .785 & .839 & .799 & \textbf{.821} \\
\midrule
\multicolumn{1}{l}{\textbf{Overall mean}} &   &   &   &   &   &   & \cellcolor{black!8}\textbf{.833} \\
\bottomrule
\end{tabular}
\caption{\textbf{Zero-shot cross-architecture transfer.} An \textsc{Fes} probe trained on Llama-3-8B is evaluated without retraining on five other LLMs. Mean AUROC stays above 0.78 across architectures, showing that $\Phi(x)$ captures an \textit{architecture-independent} spectral signature of valid reasoning, in contrast to hidden-state probes that require per-model retraining.}
\label{tab:transfer}
\end{table}
